The Edge-transitive Polytopes that are not Vertex-transitive

In 3-dimensional Euclidean space there exist two exceptional polyhedra, the rhombic dodecahedron and the rhombic triacontahedron, the only known polytopes (besides polygons) that are edge-transitive without being vertex-transitive. We show that these polyhedra do not have higher-dimensional analogues, that is, that in dimension $d\ge 4$, edge-transitivity of convex polytopes implies vertex-transitivity. More generally, we give a classification of all convex polytopes which at the same time have all edges of the same length, an edge in-sphere and a bipartite edge-graph. We show that any such polytope in dimension $d\ge 4$ is vertex-transitive.

==> sec/zonotopes.tex <==

\section{Edge-transitive zonotopes}
\label{sec:zonotopes}

Recall the several definitions of a zonotope:

\begin{definition}
A \emph{zonotope} $Z\subset\RR^d$ is a polytope which satisfies any of the following properties:
%
\begin{myenumerate}
	\item $Z$ is the projection of a $d$-cube,
	\item $Z$ has only centrally symmetric faces,
	\item $Z$ has only centrally symmetric 2-faces,
	\item $Z$ can be written as the Minkowski sum of line segments.
\end{myenumerate}
\end{definition}

We give a full classification of the edge-transitive zonotopes, which will turn out to be the following:

\begin{theorem}\label{res:edge_transitive_zonotopes}
If $Z\subset\RR^d$ is an edge-transitive zonotope, then $Z$ is one of the following:
%
\begin{myenumerate}
	\item a regular $2k$-gon,
	\item a certain non-regular $4k$-gon,
	\item a $d$-cube,
	\item a $(2k,\...,2k)$-hyperprism, that is, the $k$-fold cartesian product of the regular $2k$-gon with itself,
	\item the rhombic dodecahedron, or
	\item the rhombic triacontahedron.
\end{myenumerate}
\end{theorem}

While the $(4,...,4)$-hyperprism is also just the $d$-cube for an appropriate \emph{even} $d\ge 2$, the $d$-cubes actually exist also in odd dimensions and are therefore listed separately.

The theorem follows from the following observation.

\begin{proposition}\label{res:edge_transitive_permutahedra}
If $P\subseteq\RR^d$ is an edge-transitive $\Gamma$-permutahedron, then $P$ is one of the following:
%
\begin{myenumerate}
	\item a $d$-cube,
	\item a $(2k,\...,2k)$-hyperprism.
\end{myenumerate}
%
\begin{proof}
	\TODO
\end{proof}
\end{proposition}

\begin{proof}[Proof of \cref{res:edge_transitive_zonotopes}]
\TODO
\end{proof}

